Bias in Unsupervised Anomaly Detection in Brain MRI

Unsupervised anomaly detection methods offer a promising and flexible alternative to supervised approaches, holding the potential to revolutionize medical scan analysis and enhance diagnostic performance. In the current landscape, it is commonly assumed that differences between a test case and the training distribution are attributed solely to pathological conditions, implying that any disparity indicates an anomaly. However, the presence of other potential sources of distributional shift, including scanner, age, sex, or race, is frequently overlooked. These shifts can significantly impact the accuracy of the anomaly detection task. Prominent instances of such failures have sparked concerns regarding the bias, credibility, and fairness of anomaly detection. This work presents a novel analysis of biases in unsupervised anomaly detection. By examining potential non-pathological distributional shifts between the training and testing distributions, we shed light on the extent of these biases and their influence on anomaly detection results. Moreover, this study examines the algorithmic limitations that arise due to biases, providing valuable insights into the challenges encountered by anomaly detection algorithms in accurately learning and capturing the entire range of variability present in the normative distribution. Through this analysis, we aim to enhance the understanding of these biases and pave the way for future improvements in the field. Here, we specifically investigate Alzheimer's disease detection from brain MR imaging as a case study, revealing significant biases related to sex, race, and scanner variations that substantially impact the results. These findings align with the broader goal of improving the reliability, fairness, and effectiveness of anomaly detection in medical imaging.

==> 3_3_bias_in_the_wild.tex <==
\subsection{Optional: Detection Performance in the Wild} 
Would be an interesting experiment since in~\autoref{sec::bias} the setup is very controlled for, i.e., only train on white female, Siemens, 3T, which might not appear in realistic scenarios where the datasets are more mixed (at least for the sex shift). However, there might be space limitations due to everything else we want to show. 
\cosmin{Aim: Check if these biases occur in a 'real-life' setup, where we train on the whole IXI dataset}
In this section, we performed experiments, following the common approach of utilizing healthy distribution data from the IXI datasets. We conducted the same analysis as described earlier to evaluate the robustness and interpretability of the detection results.


==> 4_discussions.tex <==
\section{Discussion}
\paragraph{Scanner shifts.} The results indicate that the scanner type can introduce significant distortions in anomaly detection performance. These biases not only impact the overall error distribution (assessment bias), but also affect the ability of the methods to accurately detect Alzheimer's disease. It is essential to understand and address these scanner biases in order to develop robust and reliable anomaly detection algorithms.
\paragraph{Sex shifts.} The presence of evaluation bias masks the true performance of AD detection, particularly for male subjects. Further investigation showed that the true AD performance considerably dropped for male patients. It is essential to investigate the root of such methodological biases further and develop and bias mitigation strategies and algorithmic improvements to achieve fairer and more reliable detection of anomalies across different sex groups.
